The Sense of Logging in the Linux Kernel

Logging plays a crucial role in software engineering because it is key to perform various tasks including debugging, performance analysis, and detection of anomalies. Despite the importance of log data, the practice of logging still suffers from the lack of common guidelines and best practices. Recent studies investigated logging in C/C++ and Java open-source systems. In this paper, we complement these studies by conducting the first empirical study on logging practices in the Linux kernel, one of the most elaborate open-source development projects in the computer industry. We analyze 22 Linux releases with a focus on three main aspects: the pervasiveness of logging in Linux, the types of changes made to logging statements, and the rationale behind these changes. Our findings show that logging code accounts for 3.73% of the total source code in the Linux kernel, distributed across 72.36% of Linux files. We also found that the distribution of logging statements across Linux subsystems and their components vary significantly with no apparent reasons, suggesting that developers use different criteria when logging. In addition, we observed a slow decrease in the use of logging-reduction of 9.27% between versions v4.3 and v5.3. The majority of changes in logging code are made to fix language issues, modify log levels, and upgrade logging code to use new logging libraries, with the overall goal of improving the precision and consistency of the log output. Many recommendations are derived from our findings such as the use of static analysis tools to detect log-related issues, the adoption of common writing styles to improve the quality of log messages, the development of conventions to guide developers when selecting log levels, the establishment of review sessions to review logging code, and so on. [...]

==> sec-background.tex <==
\section{Background}\label{sec:background}
In this section, we present an overview of the Linux kernel project, its structure, the logging libraries used by Linux developers, and how logging in Linux is different from other projects written in C/C++.

\subsection{The Linux Kernel}
The Linux kernel is a free and open-source software distributed under the GPLv2\footnote{\url{https://www.gnu.org/licenses/old-licenses/gpl-2.0.html}} license. It is responsible for managing the interactions between hardware components and the higher-level programs that make use of them. Used across a wide range of computer systems, from mobile devices and server systems to supercomputers, the kernel can be considered as one of the most important software components in the computing industry. In fact, we are surrounded by the Linux kernel in one way or another. Being developed by roughly fifteen thousand developers throughout its history, as of 2020, it contains around 18M lines of C code. This project is continuously evolving in order to meet both hardware manufacturers' requirements and end-user expectations. In its version 5.3, the Linux kernel received 14,605 commits from 1,881 developers, adding 837,732 and removing 253,255 lines of code, which represents an increase of 584,477 lines of code when compared to its previous version.~\footnote{\url{https://github.com/gregkh/kernel-history/}}

The Linux kernel consists of five major subsystems\footnote{\url{https://github.com/gregkh/kernel-history/blob/master/scripts/genstat.pl}}; each of them covering particular aspects of the project. Table~\ref{tbl:subsystems} shows the system decomposition. The \emph{core} subsystem is in charge of memory management, inter-process communication, management of I/O operations, among others. The \emph{filesystem} subsystem is responsible for providing the file system interface as well as individual file system implementations. The \emph{drivers} subsystem provides device and sound drivers as well as the implementation of cryptography algorithms used within the system and other security-related code. Finally, the \emph{net} and \emph{arch} subsystems are responsible for networking and architecture-specific code, respectively. In the following sections, we frequently refer to these subsystems while discussing our results.

\begin{table}[!htbp]
 \caption{Linux kernel architectural decomposition}\label{tbl:subsystems}
 \centering
 \begin{tabular}{lr}
 \toprule
 \textbf{Subsystem} & \textbf{Top level directories} \\ \midrule
 \emph{core} & init, block, ipc, kernel, lib, mm, virt \\
 \emph{filesystem} & fs \\
 \emph{drivers} & crypto, drivers, sound, security \\
 \emph{net} & net \\
 \emph{arch} & arch \\ \bottomrule
 \end{tabular}
\end{table}

\subsection{Logging in the Linux kernel}
Log messages are used to record relevant information about a running system. These messages usually comprise three elements: (i) the \emph{log level} of the event being recorded; (ii) a \emph{static message} that describes that event; and, optionally, (iii) \emph{variables} related to the logged event. A log message is typically generated by the execution of a function specifically created for that purpose. These functions can be either project-specific or provided by external logging libraries and frameworks.

The Linux kernel provides to developers its own set of logging functions. One of the simplest ways to write a message to the kernel log buffer is by using the \texttt{printk()} function. It is the kernel's equivalent of \texttt{printf()}, with the difference that it allows developers to specify the log level of the event being recorded~\citep{corbet2005linux}. An example of a log statement is as follows:

\begin{verbatim}
  printk(KERN_ERR "Device initialized with return code %d\n", code);
\end{verbatim}

\noindent where \texttt{KERN\_ERR} corresponds to the log level, \texttt{"Device initialized with return code \%d\textbackslash n"} is the static message, and \texttt{code} is the corresponding variable.

There are eight log levels defined in the Linux kernel, representing different degrees of severity (see  Table~\ref{tbl:loglevels}). \texttt{KERN\_WARNING} is the default log level and is assigned to a message in case no log level is specified when calling \texttt{printk()}.

\begin{table}[th]
    \caption{The eight possible log levels defined in the Linux kernel.} \label{tbl:loglevels}
    \centering
    \begin{tabular}{ll}
        \toprule
        \textbf{Log level} & \textbf{Description} \\ \midrule
         \texttt{KERN\_EMERG} & System is unusable \\
         \texttt{KERN\_ALERT} & An action must be taken immediately \\
         \texttt{KERN\_CRIT} & Critical conditions \\
         \texttt{KERN\_ERR} & Error conditions \\
         \texttt{KERN\_WARNING} & Warning conditions \\
         \texttt{KERN\_NOTICE} & Normal but significant condition \\
         \texttt{KERN\_INFO} & Informational \\
         \texttt{KERN\_DEBUG} & Debug-level messages \\ \bottomrule
    \end{tabular}
\end{table}

Additional sets of logging functions were introduced in the Linux kernel v1.3.983 with the aim of making logging statements more concise. These functions incorporate log levels in their names. Therefore, in order to log a debug or informational message, instead of using the \texttt{printk()} function with the \texttt{KERN\_DEBUG} and \texttt{KERN\_INFO} levels as parameters, developers can use the \texttt{pr\_debug()} and \texttt{pr\_info()} functions, respectively. Another family of functions specifically designed for device drivers, e.g.\ \texttt{dev\_dbg()} and \texttt{dev\_info()}, automatically include device names in their outputs, making it easier to identify where log messages are originated from. Table~\ref{tbl:printk-helpers} lists both sets of functions and their corresponding log levels. Currently, some kernel components present their own logging functions, which are able to generate messages with service-specific information. Examples include network device and TI wl1251 drivers, which provide the \texttt{netdev\_*()} and \texttt{wl1251\_*()} families of logging functions, respectively.

\begin{table}[th]
    \caption{New sets of logging functions.}
    \label{tbl:printk-helpers}
    \centering
    \begin{tabular}{lll}
        \toprule
        \textbf{Log level} & \textbf{\texttt{pr\_*()} function} & \textbf{\texttt{dev\_*()} function} \\ \midrule
        \texttt{KERN\_EMERG} & \texttt{pr\_emerg()} & \texttt{dev\_emerg()} \\
         \texttt{KERN\_ALERT} & \texttt{pr\_alert()} & \texttt{dev\_alert()} \\
         \texttt{KERN\_CRIT} & \texttt{pr\_crit()} & \texttt{dev\_crit()} \\
         \texttt{KERN\_ERR} & \texttt{pr\_err()} & \texttt{dev\_err()} \\
         \texttt{KERN\_WARNING} & \texttt{pr\_warn()} & \texttt{dev\_warn()} \\
         \texttt{KERN\_NOTICE} & \texttt{pr\_notice()} & \texttt{dev\_notice()} \\
         \texttt{KERN\_INFO} & \texttt{pr\_info()} & \texttt{dev\_info()} \\
         \texttt{KERN\_DEBUG} & \texttt{pr\_debug()} & \texttt{dev\_dbg()} \\ \bottomrule
    \end{tabular}
\end{table}

%\spverb|dev_*()| functions, which are defined for device drivers, are another set of functions that also includes the loglevel in the function name itself. These functions automatically include the device name in the output, making it easy to see where the messages originated from. The only benefits these new macros serve are conciseness over \printk and dynamic debugging. 

%Nowadays, inspired by \spverb|pr_*()| and \spverb|dev_*()|, today specific services such as network device drivers (\spverb|netdev_*()|) and v4l2 drivers (\spverb|vl42_*()|) have now defined helpers macros that include a unique prefix consisting of the driver name and other service-specific debug information.

% DataReference - https://www.linuxfoundation.org/press-release/2017/10/linux-foundation-releases-annual-kernel-development-report/ this link says its more than fifteen thousand}
